Meta-Gradients in Non-Stationary Environments

Meta-gradient methods (Xu et al., 2018; Zahavy et al., 2020) offer a promising solution to the problem of hyperparameter selection and adaptation in non-stationary reinforcement learning problems. However, the properties of meta-gradients in such environments have not been systematically studied. In this work, we bring new clarity to meta-gradients in non-stationary environments. Concretely, we ask: (i) how much information should be given to the learned optimizers, so as to enable faster adaptation and generalization over a lifetime, (ii) what meta-optimizer functions are learned in this process, and (iii) whether meta-gradient methods provide a bigger advantage in highly non-stationary environments. To study the effect of information provided to the meta-optimizer, as in recent works (Flennerhag et al., 2021; Almeida et al., 2021), we replace the tuned meta-parameters of fixed update rules with learned meta-parameter functions of selected context features. The context features carry information about agent performance and changes in the environment and hence can inform learned meta-parameter schedules. We find that adding more contextual information is generally beneficial, leading to faster adaptation of meta-parameter values and increased performance over a lifetime. We support these results with a qualitative analysis of resulting meta-parameter schedules and learned functions of context features. Lastly, we find that without context, meta-gradients do not provide a consistent advantage over the baseline in highly non-stationary environments. Our findings suggest that contextualizing meta-gradients can play a pivotal role in extracting high performance from meta-gradients in non-stationary settings.

==> core/tables.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf Method} &\multicolumn{1}{c}{\bf Total Reward ($\alpha_e$)}  &\multicolumn{1}{c}{\bf Total Reward ($\alpha_e$, $\alpha_{l_2}$)}
\\ \hline \\
AC              &   1.24(0.09)  &  1.61(0.03)  \\
AC, MG          &   1.29(0.08)  &  1.09(0.21) \\
AC, BMG         &   1.32(0.08)  &  1.47(0.17) \\
AC, SMG-reward  &   1.58(0.06)  &  1.77(0.11) \\
AC, SMG-rich*   &   1.62(0.10)  &  1.53(0.24) \\
AC, SBMG-reward &   1.74(0.03)  &  0.36(0.13) \\
AC, SBMG-rich   &   \textbf{1.79(0.07)}  &  \textbf{2.06(0.06)} \\
\end{tabular}
\caption{Two Colors Environment with Actor-Critic Agent. Comparison of total returns over 10 random seeds.}
\label{tab:two_colors_ac}
\end{center}
\end{table}


\begin{table}[t]
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf Method}  &\multicolumn{1}{c}{\bf Total Reward (M)}
\\ \hline \\
Q-lambda              &  0.58(0.07) \\
Q-lambda, BMG         &  1.78(0.03) \\
Q-lambda, SBMG-reward &  \textbf{1.93(0.03)} \\
\end{tabular}
\caption{Two Colors Environment with $Q(\lambda)$ Agent. Comparison of total returns over 10 random seeds.}
\label{tab:two_colors_ql}
\end{center}
\end{table}


\begin{table}[t]
\begin{center}
\begin{tabular}{lll}
\multicolumn{1}{c}{\bf Method}  &\multicolumn{1}{c}{\bf Total Reward (4 MDPs)} &\multicolumn{1}{c}{\bf Total Reward (1k MDPs)}
\\ \hline \\
Q-lambda              &  14.77 (1.78) & 12.03 (0.96) \\
Q-lambda, BMG         &  14.79 (1.56) & 11.71 (0.71) \\
Q-lambda, SBMG-reward &  15.00 (2.21) & 13.36 (0.68) \\
Q-lambda, SBMG-rich*  &  \textbf{16.03 (1.40)} & \textbf{13.63 (0.64)} \\
\end{tabular}
\caption{Switching MDP with Q-Lambdawith $Q(\lambda)$ Agent. Comparison of total returns over 10 random seeds.}
\label{tab:switching_mdp_ql}
\end{center}
\end{table}


